Self-supervised Answer Retrieval on Clinical Notes

Retrieving answer passages from long documents is a complex task requiring semantic understanding of both discourse and document context. We approach this challenge specifically in a clinical scenario, where doctors retrieve cohorts of patients based on diagnoses and other latent medical aspects. We introduce CAPR, a rule-based self-supervision objective for training Transformer language models for domain-specific passage matching. In addition, we contribute a novel retrieval dataset based on clinical notes to simulate this scenario on a large corpus of clinical notes. We apply our objective in four Transformer-based architectures: Contextual Document Vectors, Bi-, Poly- and Cross-encoders. From our extensive evaluation on MIMIC-III and three other healthcare datasets, we report that CAPR outperforms strong baselines in the retrieval of domain-specific passages and effectively generalizes across rule-based and human-labeled passages. This makes the model powerful especially in zero-shot scenarios where only limited training data is available.

==> Appendices.tex <==

\begin{table}[h!]
%\begin{SCtable}
\centering
 \begin{tabular}{l c c c} 
 \textbf{Experiment} & \textbf{R@1} & \textbf{R@10} & \textbf{R@32} \\
 \hline
 \hline

\textbf{Precomputed Embeddings} \\
CDV+BioBERT (Replication)                       & 62.36          & 96.0           & \textbf{100} \\
CDV+FastText (Replication)                      & 60.49          & \textbf{98.37} & 99.9 \\
\hline
\textbf{BioBERT Fine-Tuning} \\
CDV+BioBERT FT (Non-Incremental)                & 10.5           & 93.6           & 99.9 \\
CDV+BioBERT FT(Multi-CLS)                       & 49.9           & 94.6           & 99.9 \\
CDV+BioBERT FT(Multi-CLS) + FF-Pool             & 58.4           & 95.4           & 99.9 \\
CDV+BioBERT FT(CLS-Pool) + ELU                  & 64.5           & 96.4           & \textbf{100}  \\ 
CDV+BioBERT FT(CLS) + LAMB-Optim + LR-Decr.     & 61.2           & 98.3           & 99.9 \\

\hline
\textbf{Different Pooling Strategies} \\
CDV+BioBERT 4 Last Layer Pool (256-BLSTM)       & 47.0           & 94.0           & 99.9 \\
CDV+BioBERT 4 Last Layer Pool (512-BLSTM)       & 51.59          & 94.47          & 99.9 \\
CDV+BioBERT AVG-Pool+ELU (512-BLSTM)            & 61.5           & 96.3           & \textbf{100}  \\

\hline
\textbf{Without LSTM} \\
BioBERT AVG without LSTM                        & 50.5           & 94.5           & 99.9 \\

\hline
\textbf{Hierarchical RNN} \\
CDV+FastText (Word GRU + BiLSTM)                & 10.0           & 93.9           & 99.9 \\
CDV+FastText (Word GRU + BiLSTM) + Noise        & 11.31          & 94.99          & 99.9 \\ 

\hline
\textbf{LSTM Replacement with a Transformer} \\
CDV-Transformer CLS-Pool 4-Layer 6-Heads BS64   & 53.3           & 95.0           & 99.9 \\
CDV-Transformer CLS-Pool 6-Layer 8-Heads BS48   & 53.5           & 95.2           & 99.9 \\
CDV-Transformer AVG-Pool 6-Layer 8-Heads BS48   & 58.0           & 95.8           & 99.9 \\
CDV-Transformer FT(CLS-Pool) 4-Layer 6-Heads    & 63.2           & 96.2           & 99.9 \\
CDV-Transformer FT(CLS-Pool) 6-Layer 8-Heads    & 60.4           & 96.1           & 99.9 \\

\end{tabular}

\caption{Hyperparameters}
\label{fig:cdv_enhancements}
 

%\end{SCtable}
\end{table}

==> __latexindent_temp.tex <==
\section{Introduction}

Open-ended search intentions, such as questions about health, often lead to complex answers that span multiple sentences (see \autoref{fig:doc_visualization}). These passages are often embedded in the context of long documents, where multiple latent query-related aspects might be discussed. Retrieving such non-factoid answers from a large corpus of passages is a complex task that requires semantic understanding of discourse and document context \cite{arora2016latent, nanni2017benchmark, cohan2018discourse}. Traditional retrieval methods often assume that answer passages are independent and retrieve them using term matching \cite{o1980answer, salton1993approaches} or learn to rank them using human-annotated query--answer pairs as training data \cite{tellex2003quantitative, yang2016beyond, zhu2019hierarchical}. More recent approaches aim to find passages in the context of longer documents \cite{keikha2014retrieving, arnold2019sector} and utilize hierarchical attention \cite{zhu2019hierarchical} or latent neural representations \cite{arnold2020learning} for retrieving them with high recall.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Graphics/IJCNLP_Fig_1.pdf}
    \caption{Application of CAPR showing three relevant retrieval results of MIMIC-III passages (blue) for a query (yellow) involving the entity ``Cardiomyopathy'' and the latent clinical aspect ``Family History''.}
    \label{fig:doc_visualization}
\end{figure}

A major challenge in this scenario is to apply neural contextual architectures for ad-hoc retrieval from large datasets with low latency. Typically, the Cross-encoder architecture focuses on the interaction between query and passage at the significant cost of computation \cite{hu2014convolutional,guo2016deep,yang2016anmm}. A more efficient solution is the Bi-encoder approach, where the query is encoded independently from the passage \cite{huang2006evaluation,shen2014learning}. This model often trades speedup for retrieval accuracy. To overcome this problem, Poly-encoders combine the efficiency of Bi-encoders with the effectiveness from additional interaction features \cite{humeau2020polyencoders}.

\paragraph{Our contribution.} 
We approach the task of retrieving answer passages for doctors, who search for clinical manifestations in thousands of health records. Our setup resembles the clinical back\-ground--fore\-ground scenario \cite{cheng2004study}, where a query focuses on an \emph{entity} (e.g., a disease or health problem) and a specific \emph{aspect} of the entity (e.g., its anamnesis or pathology, see \autoref{fig:doc_visualization}). This is especially challenging because in this domain, there is no task-specific training data available. The main contributions of this paper include:
\begin{itemize} 
\item We introduce Clinical Answer Passage Retrieval\footnote{Code and evaluation data available at [ANONYMIZED]} (CAPR), a novel training objective that allows self-supervised fine-tuning of language models, such as BioBERT \cite{lee2019biobert}. We apply CAPR in four recent Transformer-based architectures: Contextual Discourse Vectors (CDV), Cross-encoder, Bi-encoder and Poly-encoder.
\item Our method requires no external labels as training data. Instead, we utilize features extracted from Named Entity Recognition (NER) and corpus-specific rules. This enables us to train self-supervised, using in-domain unlabeled clinical data.
\item We apply CAPR in a clinical answer passage retrieval scenario on 7.4k clinical notes from MIMIC-III and evaluate it on three additional human annotated healthcare datasets: WikiSectionQA, MedQuAD and HealthQA.
\item Our experiments show that CAPR significantly increases cross-domain retrieval performance with up to 72.9\% Recall@1 on MIMIC-III. This is a 15.7 points increase compared to fine-tuning CDV+BioBERT on the same task.
\end{itemize}
While Poly-encoders have shown significant improvements in document retrieval, this paper is the first to utilize this architecture in a self-supervised answer retrieval task. 

%This is especially helpful for the training for retrieval models in specialised domains, such as clinical care.

%In summary, the main contributions of this paper include:
%\begin{itemize}
%    \item We compare three representation based and one end to end trained architecture on the passage retrieval task. We examine them in terms of performance on the task and give insights into their real world applicability with regard to computational efficiency.
%    \item We introduce a new dataset based on MIMIC-III. The dataset contains entity- and aspect-annotations that can be used for training and evaluation on the passage retrieval and passage ranking task.
%    \item We show, that fine-tuning neural Transformer based generalized language models on a passage ranking task increases the generalization capability of the models. Furthermore, this decreases the required amount and quality of the used training data in comparison to the LSTM based CDV architecture.
%    \item We show that fine-tuning the underlying language model of CDV does not improve the models performance on the passage ranking task. We use multiple fine-tuning strategies and show that no model with a fine-tuned sentence encoder outperforms the baseline.
%    \item We evaluate all of our proposed methods in extensive experiments on four english healthcare evaluation datasets in a zero shot passage ranking task.
%\end{itemize}

This paper is structured as follows: We overview related work in Section \ref{sec:relatedwork}. We introduce our approach in Section \ref{sec:method}. In Section \ref{sec:evaluation} we present our experimental evaluation and a deep error analysis. In Section \ref{sec:conclusion}, we draw a conclusion.


==> tables.tex <==
\begin{table*}
\centering

 \begin{tabular}{l c c c} 
 \textbf{Experiment} & \textbf{R@1} & \textbf{R@10} & \textbf{R@32} \\
 \hline
 \hline
\textbf{Reported CDV Performance} \\
CDV+BioBERT (Paper)                             & \textbf{65.21} & 97.84          & -  \\ 
CDV+FastText (Paper)                            & 60.34          & 97.49          & -  \\

\hline
\textbf{Replications} \\
CDV+BioBERT (Replication)                       & 62.36          & 96.0           & \textbf{100} \\
CDV+FastText (Replication)                      & 60.49          & \textbf{98.37} & 99.9 \\
\hline
\textbf{BioBERT Fine-Tuning} \\
CDV+BioBERT FT (Non-Incremental)                & 10.5           & 93.6           & 99.9 \\
CDV+BioBERT FT(Multi-CLS)                       & 49.9           & 94.6           & 99.9 \\
CDV+BioBERT FT(Multi-CLS) + FF-Pool             & 58.4           & 95.4           & 99.9 \\
CDV+BioBERT FT(CLS-Pool) + ELU                  & 64.5           & 96.4           & \textbf{100}  \\ 
CDV+BioBERT FT(CLS) + LAMB-Optim + LR-Decr.     & 61.2           & 98.3           & 99.9 \\

\hline
\textbf{Different Pooling Strategies} \\
CDV+BioBERT 4 Last Layer Pool (256-BLSTM)       & 47.0           & 94.0           & 99.9 \\
CDV+BioBERT 4 Last Layer Pool (512-BLSTM)       & 51.59          & 94.47          & 99.9 \\
CDV+BioBERT AVG-Pool+ELU (512-BLSTM)            & 61.5           & 96.3           & \textbf{100}  \\

\hline
\textbf{Without LSTM} \\
BioBERT AVG without LSTM                        & 50.5           & 94.5           & 99.9 \\

\hline
\textbf{Hierarchical RNN} \\
CDV+FastText (Word GRU + BiLSTM)                & 10.0           & 93.9           & 99.9 \\
CDV+FastText (Word GRU + BiLSTM) + Noise        & 11.31          & 94.99          & 99.9 \\ 

\hline
\textbf{LSTM Replacement with a Transformer} \\
CDV-Transformer CLS-Pool 4-Layer 6-Heads BS64   & 53.3           & 95.0           & 99.9 \\
CDV-Transformer CLS-Pool 6-Layer 8-Heads BS48   & 53.5           & 95.2           & 99.9 \\
CDV-Transformer AVG-Pool 6-Layer 8-Heads BS48   & 58.0           & 95.8           & 99.9 \\
CDV-Transformer FT(CLS-Pool) 4-Layer 6-Heads    & 63.2           & 96.2           & 99.9 \\
CDV-Transformer FT(CLS-Pool) 6-Layer 8-Heads    & 60.4           & 96.1           & 99.9 \\

\end{tabular}

\caption{Results of the CDV Enhancement Approaches}
\label{fig:cdv_enhancements}
 

\end{table*}
